The stable converse soul question for positively curved homogeneous spaces

The stable converse soul question (SCSQ) asks whether, given a real vector bundle \(E\) over a compact manifold, some stabilization \(E\times\R^k\) admits a metric with non-negative (sectional) curvature. We extend previous results to show that the SCSQ has an affirmative answer for all real vector bundles over any simply connected homogeneous manifold with positive curvature, except possibly for the Berger space \(B^{13}\). Along the way, we show that the same is true for all simply connected homogeneous spaces of dimension at most seven, for arbitrary products of simply connected compact rank one symmetric spaces of dimensions multiples of four, and for certain products of spheres. Moreover, we observe that the SCSQ is "stable under tangential homotopy equivalence": if it has an affirmative answer for all vector bundles over a certain manifold \(M\), then the same is true for any manifold tangentially homotopy equivalent to~\(M\). Our main tool is topological K-theory. Over \(B^{13}\), there is essentially one stable class of real vector bundles for which our method fails.

==> WallachFlag.tex <==
In this section we prove that $\alpha_O$ is surjective for the usual presentations of the Wallach flag manifolds $W^{12}=\Sp(3)/\Sp(1)^3 $ and $W^{24}= F_4/\Spin(8)$ (the case $W^6$ is treated in \cref{S: Homogeneous spaces of dimension 7}). This gives \cref{THM: SCST for homogeneous of positive curvature} for these spaces as a consequence of \cref{PROP: surjectivity of alphaO implies SISC}.

In contrast to the case $W^6$, for $W^{12}$ and $W^{24}$ the realification map $\rx: K\to KO$ is not surjective, and various observations are needed in order to obtain the surjectivity of $\alpha_O$ from that of $\alpha$.
The cohomology of the Wallach spaces $W^{6i}$ (where $i=1,2,4$) is well known (see for example \cite{AZ:Geometrically}):
\[
H^k(W^{6i},\Z) =
\begin{cases}
  \Z & \text{ if $k=0,6i$,}                                                                        \\
  \Z\oplus\Z  & \text{ if $k=2i,4i$,}
\\
  0 & \text{ otherwise.}
\end{cases}
\]
The KO-theory of $W^{12}$ and $W^{24}$ can be computed from the following result.

\begin{lem}\label{L: lemma 2.5 hoggar}
Suppose $M$ is a compact (Hausdorff) space whose integral cohomology is (finitely generated) free and concentrated in dimensions multiples of 4. Denote by $b_k$ the rank of the group $H^k(M,\Z)$.  Then
\begin{align*}
KO^0 (M) = KO^{-4} (M) &= \left( b_0 + b_4 + b_8+\dots\right)\Z,  \\
KO^{-2} (M) = KO^{-1} (M) &= \left(  b_0 + b_8 + b_{16}+\dots \right)\Z_2, \\
KO^{-6} (M) = KO^{-5} (M) &= \left(  b_4 + b_{12} + b_{20}+\dots \right)\Z_2, \\
KO^{-3} (M) = KO^{-7} (M) &= 0.
\end{align*}
\end{lem}

\begin{rem}
\Cref{L: lemma 2.5 hoggar}  is very similar to Lemma 2.5 in Hoggar's article \cite{Hoggar:onKO}, where the hypotheses are given in terms of the cell structure of $M$. However, Hoggar's proof still works in our setting, and it is a simple spectral sequence argument.
\end{rem}

\subsubsection{The Wallach flag manifold of dimension 12}\label{SS: W12}

This is the homogeneous space \(\Sp(3)/\Sp(1)^3\) given by the obvious diagonal block inclusion \(i\colon \Sp(1)^3\to \Sp(3)\).
The complex representation rings of the groups involved in \(W^{12}\) are the polynomial rings (see \cite{BtD:Lie})
\[
R(\Sp(3))= \Z [\Lambda^1 , \Lambda^2, \Lambda^3 ],\qquad R(\Sp(1)^3) = R(\Sp(1))^{\otimes 3} = \Z [x_1 ,x_2, x_3 ].
\]
\PRELIM{I already defined real and quaternionic type in section 3.2}Here $x_i$ denotes the representation of quaternionic type of complex rank $2$ generating each factor $R(\Sp(1))$.
\COMMENT[DG]{You wrote ``Each $x_i$ has trivial determinant''- what does this mean exactly? You also wrote ``As the $x_i$ have trivial determinants, the images of the exterior powers $\Lambda^i$ can be computed as follows:''}

\COMMENT[DG]{Reference? You sent me one with $\lambda$-rings}It is straightforward to compute the restriction of representations $i^*: R(\Sp(3))\to R(\Sp(1)^3)$:
\begin{align*}
i^* (\Lambda^1 ) &= x_1 + x_2 + x_3\\
i^* (\Lambda^2 ) &= x_1 x_2 + x_1 x_3 + x_2 x_3 + 3\\
i^* (\Lambda^3 ) &= 2( x_1 + x_2 + x_3 ) + x_1 x_2 x_3
\end{align*}
Denote by $y_i$ the reduced element $\alpha(x_i - 2)$. Hodgkin's theorem yields:\COMMENT[DG]{Reference for Hodgkin's theorem? Probably we include it in the IMPROVE PITTIE part}
\begin{equation}
K(W^{12}) = \Z [y_1 , y_2, y_3 ] / ( y_1 + y_2 + y_3 , y_1 y_2 + y_1 y_3 + y_2 y _3 , y_1 y_2 y_3 )
\end{equation}
In other words, $K(W^{12})$ is the coinvariant algebra of the symmetric group $S_3$ acting by permutations on $\Z [y_1 , y_2, y_3 ]$.  It is free abelian of rank $6$, and an explicit basis is well known\COMMENT[DG]{Reference needed? In [Notes]}:
\begin{equation}\label{EQ: additive basis of K(W12)}
1 , y_2 , y_1 y_3 , y_2 y_3^2 , y_2 y_3 , y_3
\end{equation}
By \cref{L: lemma 2.5 hoggar} we have that $KO^1 (W^{12}) = 0$ and $KO^2 (W^{12}) = \Z_2\oplus\Z_2\oplus\Z_2 = (\Z_2)^3$, and the Bott sequence therefore yields an exact sequence:
\[
 0 \to KO(W^{12}) \xrightarrow{\cx} K(W^{12}) \to (\Z_2)^3  \to 0
\]

Since the product of representations of quaternionic type is of real type, the elements $1, y_1 y_3$ and $y_2 y_3$ of the additive basis \eqref{EQ: additive basis of K(W12)} lie in $KO(W^{12})$, i.e., we have that $1=\cx(e_1), y_1 y_3=\cx(e_2), y_2 y_3=\cx(e_3)$ for some $e_1=1, e_2,e_3\in KO(W^{12})$.

The remaining basis elements \(q_1:=y_2, q_2:=y_2 y_3^2,q_3:=y_3\) lie in the image of \(\cx'\colon  KSp(W^{12})\to K(W^{12})\). In particular, \(\cx\circ\rx(q_i) = q_i + \tx(q_i) = 2q_i\).

Now let $KO'\subset KO(W^{12})$ be the subgroup generated by $e_1, e_2, e_3, \rx(q_1), \rx(q_2), \rx(q_3)$. Then $K(W^{12})/\cx(KO')$ is isomorphic to $(\Z_2)^3 =K(W^{12})/\cx(KO(W^{12}))$. Since $\cx$ is injective in this case, we have that $KO' = KO(W^{12})$. Now each of the basis elements $e_1, e_2, e_3, \rx(q_1), \rx(q_2), \rx(q_3)$ lies in the image of $RO(\Sp(1)^3)$ by $\alpha_O$, so we are done.

\qed

\subsubsection{The Wallach flag manifold of dimension 24}\label{SS: W24}

The Wallach flag manifold $W^{24}$ is the homogeneous space $F_4/\Spin(8)$. Consider the commutative diagram
\[
\xymatrix{  RO(\Spin(8))\ar[d]^{\cx}\ar[r]^{\alpha_0} & KO(W^{24})\ar[d]^{\cx}\\
R(\Spin(8))\ar[r]^{\alpha}  & K(W^{24})}
\]
The surjectivity of $\alpha_O$ is an immediate consequence of the following three facts.
\begin{itemize}
\item $\alpha$ is surjective, which follows directly from \cref{Improvement pf Pittie's}.
\item $\cx:RO(\Spin(8))\to R(\Spin(8))$ is an isomorphism. For a Lie group, complexification is always injective. The surjectivity follows from the explicit description of $R(\Spin(8))$: it is the polynomial ring
\[
R(\Spin(8))=\Z [\Lambda^1,\Lambda^{2},\Delta_{+},\Delta_{-}],
\]
where the representations $\Lambda^1,\Lambda^{2},\Delta_{+},\Delta_{-}$ are of real type (see \cite{BtD:Lie}).

\item  $\cx: KO(W^{24})\to K(W^{24})$ is an isomorphism. This follows directly from the Bott sequence, since $KO^1(W^{24})=KO^2(W^{24})=0$ by \cref{L: lemma 2.5 hoggar}.
\end{itemize}

\qed

